Visual Graphs from Motion (VGfM): Scene understanding with object geometry reasoning

Recent approaches on visual scene understanding attempt to build a scene graph -- a computational representation of objects and their pairwise relationships. Such rich semantic representation is very appealing, yet difficult to obtain from a single image, especially when considering complex spatial arrangements in the scene. Differently, an image sequence conveys useful information using the multi-view geometric relations arising from camera motion. Indeed, in such cases, object relationships are naturally related to the 3D scene structure. To this end, this paper proposes a system that first computes the geometrical location of objects in a generic scene and then efficiently constructs scene graphs from video by embedding such geometrical reasoning. Such compelling representation is obtained using a new model where geometric and visual features are merged using an RNN framework. We report results on a dataset we created for the task of 3D scene graph generation in multiple views.

==> macros3.tex <==
%\input{local-definitions}
\newcommand{\trinv}{\mbox{$^{\top\,-1}$}}
\newcommand{\mtr}{\mbox{$^{-\top}$}}
\newcommand{\rank}{\mbox{\rm rank}}
\newcommand{\sign}{\mbox{\rm sign}}
\newcommand{\diag}{\mbox{\rm diag}}
\newcommand{\med}{\mbox{\rm med}} % maybe change/drop this
\newcommand{\adj}{\mbox{$^*$}}
\def\ijk{_i^{jk}}
\def\Tri{{\cal T}}
\def\Tijk{\Tri\ijk}

% Real and complex numbers
\newcommand{\R}{{\cal R}}
\newcommand{\C}{{\cal C}}

% Standardized references
\newcommand{\app}[1]{appendix~\ref{app:#1}}
\newcommand{\App}[1]{Appendix~\ref{app:#1}}
\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand{\eqn}[1]{(\ref{eq:#1})}
\newcommand{\fig}[1]{Fig~\ref{fig:#1}}
\newcommand{\tab}[1]{table~\ref{tab:#1}}
\newcommand{\Tab}[1]{Table~\ref{tab:#1}}
\newcommand{\sect}[1]{section~\ref{sec:#1}}
\newcommand{\ch}[1]{chapter~\ref{ch:#1}}
\newcommand{\Ch}[1]{Chapter~\ref{ch:#1}}
\newcommand{\thm}[1]{Theorem~\ref{thm:#1}}

\newcommand{\num}[1]{(~\ref{num:#1})}
\newcommand{\Thm}[1]{Theorem~\ref{thm:#1}}
\newcommand{\pro}[1]{Proposition~\ref{pro:#1}}
\newcommand{\Pro}[1]{Proposition~\ref{pro:#1}}
\newcommand{\defn}[1]{definition~\ref{def:#1}}
\newcommand{\algo}[1]{table~\ref{alg:#1}}
\newcommand{\lem}[1]{lemma~\ref{lem:#1}}

\newcommand{\SKIP}[1]{} % Used to skip stuff we do not want type-set

%
\newcommand{\vv}[2]
   {\mbox{$
      \left(
         \begin{array}{c}
         #1 \\ #2
         \end{array}
      \right )
   $}}
%
\newcommand{\vvv}[3]
   {\mbox{$
      \left(
         \begin{array}{c}
         #1 \\ #2 \\ #3
         \end{array}
      \right )
   $}}
%
\newcommand{\vvvv}[4]
   {\mbox{$
      \left(
         \begin{array}{c}
         #1 \\ #2 \\ #3 \\ #4
         \end{array}
      \right )
   $}}
%
\newcommand{\vm}[2]
   {\mbox{$
      \left[
         \begin{array}{c}
         #1 \\ #2
         \end{array}
      \right ]
   $}}
%
\newcommand{\vvm}[3]
   {\mbox{$
      \left[
         \begin{array}{c}
         #1 \\ #2 \\ #3
         \end{array}
      \right ]
   $}}
%
\newcommand{\vvvm}[4]
   {\mbox{$
      \left[
         \begin{array}{c}
         #1 \\ #2 \\ #3 \\ #4
         \end{array}
      \right ]
   $}}
%
\newcommand{\mm}[4]
   {\mbox{$
      \left[
         \begin{array}{ccc}
         #1 & #2    \\
         #3 & #4 
         \end{array}
      \right]
   $}}
%
\newcommand{\mmm}[9]
   {\mbox{$
      \left[
         \begin{array}{ccc}
         #1 & #2 & #3   \\
         #4 & #5 & #6   \\
         #7 & #8 & #9
         \end{array}
      \right]
   $}}

%
% Quick way to do matrices
\newcommand{\mbegin} {\left [ \begin{array}}
\newcommand{\mstart} {\mbegin}
\newcommand{\mc}     {\mbegin{c}}
\newcommand{\mcc}    {\mbegin{cc}}
\newcommand{\mccc}   {\mbegin{ccc}}
\newcommand{\mcccc}  {\mbegin{cccc}}
\newcommand{\mccccc} {\mbegin{ccccc}}
\newcommand{\mend}   {\end{array} \right ]}

% Same for vectors
\newcommand{\vbegin} {\left ( \begin{array}{c}}
\newcommand{\vstart} {\vbegin}
\newcommand{\vend} {\end{array}\right )}

%
%
%
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Po}{\mbox{\({\cal P}^1\)}}
\newcommand{\PP}{\mbox{\({\cal P}^2\)}}
\newcommand{\PPP}{\mbox{\({\cal P}^3\)}}
\newcommand{\PPPPP}{\mbox{\({\cal P}^5\)}}
\newcommand{\Pn}{\mbox{\({\cal P}^n\)}}
\newcommand{\sk}[1]{[#1]_\times}
\newcommand{\bm}[1]{\mbox{\boldmath $#1$}}
%

% Stuff for doing the qed sign.
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}

\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
	\penalty50\hskip1em\null\nobreak\hfil\squareforqed
	\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

% Stuff for doing vector. NB need to not use small for lower case.
\def\vecs#1{\mathchoice%
	{\mbox{\boldmath \small $\displaystyle\bf#1$}}
	{\mbox{\boldmath \small $\textstyle\bf#1$}}
	{\mbox{\boldmath \small $\scriptstyle\bf#1$}}
	{\mbox{\boldmath \small $\scriptscriptstyle\bf#1$}}}
\def\vs#1{\protect\vecs #1}

\def\vec#1{\mathchoice%
	{\mbox{\boldmath $\displaystyle\bf#1$}}
	{\mbox{\boldmath $\textstyle\bf#1$}}
	{\mbox{\boldmath $\scriptstyle\bf#1$}}
	{\mbox{\boldmath $\scriptscriptstyle\bf#1$}}}
\def\v#1{\protect\vec #1}

% Stuff for making labels visible
\newcommand{\showlabel}[1]
	{\hskip 0.0em\marginpar{\quad\fbox{\scriptsize\rm#1}}}

\newcommand{\showeqnlabel}{
	\hbox to 0pt{\quad\quad\relax\fbox{\scriptsize\rm\eqnlblx}%
	\gdef\eqnlblx{xxxx}}} \newcommand{\eqnlblx}{}

\def\@eqnnum{\rm (\theequation)\showeqnlabel}

\newcommand{\eqnlabel}[1]{\protect\label{#1}\gdef\eqnlblx{#1}}

\newcommand{\mylabel}[1]{\label{#1}\showlabel{#1}}

\newcommand{\nofig}[1]{\centerline{\bf Figure here}}

% Stuff for doing matrix.
\def\mat#1{\mathchoice{\mbox{\boldmath$\displaystyle\tt#1$}}
	{\mbox{\boldmath$\textstyle\tt#1$}}
	{\mbox{\boldmath$\scriptstyle\tt#1$}}
	{\mbox{\boldmath$\scriptscriptstyle\tt#1$}}}
\def\m#1{\protect\mat #1}

%\newcommand{\matx}[1]{{\tt #1}}


